DLT: Conditioned layout generation with Joint Discrete-Continuous Diffusion Layout Transformer

Generating visual layouts is an essential ingredient of graphic design. The ability to condition layout generation on a partial subset of component attributes is critical to real-world applications that involve user interaction. Recently, diffusion models have demonstrated high-quality generative performances in various domains. However, it is unclear how to apply diffusion models to the natural representation of layouts which consists of a mix of discrete (class) and continuous (location, size) attributes. To address the conditioning layout generation problem, we introduce DLT, a joint discrete-continuous diffusion model. DLT is a transformer-based model which has a flexible conditioning mechanism that allows for conditioning on any given subset of all the layout component classes, locations, and sizes. Our method outperforms state-of-the-art generative models on various layout generation datasets with respect to different metrics and conditioning settings. Additionally, we validate the effectiveness of our proposed conditioning mechanism and the joint continuous-diffusion process. This joint process can be incorporated into a wide range of mixed discrete-continuous generative tasks.

==> sections/01_introduction_old.tex <==
%%%%%%%%% BODY TEXT
\section{Introduction}
An essential aspect of graphic design is layout creation: the arrangement and sizing of visual components on a canvas or document. A well-designed layout enables users to easily comprehend and efficiently interact with the information presented. The ability to generate high-quality layouts is crucial for a range of applications, including user interfaces for mobile apps and websites~\cite{RICO} and graphic design for information slides \cite{presentationSlides}, magazines \cite{MAGAZINE}, scientific papers \cite{PubLayNet}, infographics \cite{infographics}, and indoor scenes \cite{indoorScenes}.


To facilitate graphic design tasks, modelling approaches such as Generative Adversarial Networks (GANs)~\cite{LayoutGAN}, Variational Autoencoders (VAEs) \cite{LayoutVAE,VTN}, and masking completion \cite{LayoutBERT,BLT,LT} were explored to generate novel layouts. These approaches employ various architectures such as Recurrent Neural Networks (RNNs)~\cite{LayoutVAE}, Graph Neural Networks (GNNs)~\cite{LeeJELG0Y20}, and Transformers \cite{VTN,LayoutBERT,BLT,LT}. Recently proposed, Transformer-based approaches have shown to produce diverse and plausible layouts for a variety of applications and user requirements. 
 
Layouts are often represented as a set of components, each consisting of several properties, such as type, position, and size~\cite{LayoutGAN}. Recent approaches model a component as a sequence of discrete property tokens, and a layout as the concatenation of all property tokens~\cite{LayoutBERT,LT,BLT}. A transformer is then used to generate the tokens sequence. A common practice is to discretize geometry properties, such as position and size, by quantization or binning. However, using discrete tokens fails to take into account the natural representation of (geometry) data, which is continuous, and either results in poor resolution of layout composition, or in a large sparse vocabulary that is not covered well by smaller datasets.

An important aspect of layout generation is the amount of control offered to the user. We would like to allow a user to fix certain component properties, such as component type, or a set of components, and then generate the remaining properties (position and size) or components.  In transformer-based approaches, such conditioning is performed only dLayoutBERTuring inference either by masking  tokens~\cite{LayoutBERT} (non-autoregressive decoding) or by setting a prefix of components and generating more sequentially~\cite{LT,LayoutVAE} (autoregressive decoding) \elib{Elad: check if it makes sense to add refs for VTN, and BLT}. A more effective approach is to explicitly train the model to perform layout conditioning. Inspired by recent diffusion-based image editing techniques~\cite{GLIDE}, we propose a flexible editing mechanism which allows conditioning on any subset of the layout data.  We later show that this design choice improves model performance significantly compared to inference-based conditioning. 


Diffusion models are a generative approach that has gained significant attention recently. Continuous diffusion models have demonstrated remarkable generative capabilities for images~\cite{DALLE}, in terms of quality and diversity, as well as in other domains like audio \cite{diffusionSound} and video \cite{diffusionVideo}, and human motion~\cite{MDM}.
Diffusion models were extended to discrete spaces, and effectively applied to autoregressive image caption generation \cite{DISCE,DISCN}.  In fact, \cite{BLT} which extends layout transformers to enable controllability by implementing a hierarchical masking policy, can be viewed as an approximated Discrete Diffusion process.

In this paper, we introduce a Diffusion Layout Transformer (DLT) for layout generation and flexible editing.  Different from traditional layout generation models, we propose a novel framework based on a joint continuous-discrete diffusion process and provide theoretical justification for the derived optimization objective. Using a transformer-encoder architecture, we apply a diffusion process jointly both on the continuous properties of the layout components (size and location) and on the discrete ones (type). An overview of our framework is given in  Figure~\ref{fig:overview}. 

Our diffusion model addresses an important limitation of transformer-based models that solely rely on discrete layout representation, despite real layouts containing both discrete and continuous features. These models need to quantize layout data, which leads to reduced resolution and limited diversity of layout compositions. Our novelty lies in the proposed mixed discrete-continuous embedding representation and diffusion model, which as demonstrated by our comprehensive ablation study, is essential for generating high-quality layouts. Our framework offers powerful layout editing through flexible conditioning  using a condition embedding that specifies which layout properties are part of the conditioning. DLT can thus satisfy diverse controllability needs, such as unconstrained generation, generation conditioned on component properties, and layout completion.

We study the effectiveness of our DLT model by evaluating it on three popular layout datasets of diverse graphic design tasks using several common perceptual quality metrics.  Using extensive experimentation, we demonstrate that our proposed model outperforms state-of-the-art layout generative models on layout synthesis and editing tasks while maintaining runtime complexity on par with these models. By comparing different design alternatives, we show the significant contribution of both the joint diffusion process and the conditioning mechanism to the model's strong generative capabilities.

Our discrete-continuous diffusion framework has a generic design and thus can be effectively applied to other domains such as \elib{Elad: please add. Maybe include 2D/3D scene generation and remove from first paragraph|}   

%To summarize, our main contributions are:
%\begin{enumerate}
%    \item We propose a novel method for high-quality layout generation based on a joint continuous-discrete diffusion framework with powerful layout editing.
%    \item We conduct an extensive evaluation  on diverse layout benchmarks and demonstrate that our method outperforms state-of-the-art models on commonly-used quality metrics.
%\end{enumerate}


\begin{figure}[t!]
	\begin{center}
        \includegraphics[width=0.8\linewidth]{./figures/diffusion_process9.png}
    %\vspace{-10pt}
	\caption{\small{{Overview of our Joint Discrete-Continuous diffusion process for layout generation. The diffusion process is applied jointly both on the continuous attributes of the components (size and location) by adding a small Gaussian noise and on the discrete component's attribute (class) by adding a noise that adds a mass to the Mask class. The reverse diffusion model can be conditioned on any given subset of the attributes.}}}
	\label{fig:overview}
	\end{center}
\end{figure}

